Information-Theoretic Study of Time-Domain Energy-Saving Techniques in Radio Access

Reduction of wireless network energy consumption is becoming increasingly important to reduce environmental footprint and operational costs. A key concept to achieve it is the use of lean transmission techniques that dynamically (de)activate hardware resources as a function of the load. In this paper, we propose a pioneering information-theoretic study of time-domain energy-saving techniques, relying on a practical hardware power consumption model of sleep and active modes. By minimizing the power consumption under a quality of service constraint (rate, latency), we propose simple yet powerful techniques to allocate power and choose which resources to activate or to put in sleep mode. Power consumption scaling regimes are identified. We show that a ``rush-to-sleep" approach (maximal power in fewest symbols followed by sleep) is only optimal in a high noise regime. It is shown how consumption can be made linear with the load and achieve massive energy reduction (factor of 10) at low-to-medium load. The trade-off between energy efficiency (EE) and spectral efficiency (SE) is also characterized, followed by a multi-user study based on time division multiple access (TDMA).

==> Section/Ideal.tex <==
\section{Optimal Resource Allocation for Ideal Power Model}
\label{section:ideal}

\TODO{give limit capacity for infinite $T$}

\TODO{change title, not really resource allocation}

==> Section/System_power.tex <==
\section{Optimal Allocation under Power Ampliflier and Circuit Power Consumption Constraint}
\label{section:Class_A}

\TODO{talk about the non trivial dependence in the nonconvex constraint, two conflicting goals, close to saturation and low power, explain why practical power constraint promotes sparsity. Two reasons: i) load-independent and ii) load-dependent term which is concave}

\TODO{multi-user in TDMA?}
